From Counting Stations to City-Wide Estimates: Data-Driven Bicycle Volume Extrapolation

Shifting to cycling in urban areas reduces greenhouse gas emissions and improves public health. Street-level bicycle volume information would aid cities in planning targeted infrastructure improvements to encourage cycling and provide civil society with evidence to advocate for cyclists' needs. Yet, the data currently available to cities and citizens often only comes from sparsely located counting stations. This paper extrapolates bicycle volume beyond these few locations to estimate bicycle volume for the entire city of Berlin. We predict daily and average annual daily street-level bicycle volumes using machine-learning techniques and various public data sources. These include app-based crowdsourced data, infrastructure, bike-sharing, motorized traffic, socioeconomic indicators, weather, and holiday data. Our analysis reveals that the best-performing model is XGBoost, and crowdsourced cycling and infrastructure data are most important for the prediction. We further simulate how collecting short-term counts at predicted locations improves performance. By providing ten days of such sample counts for each predicted location to the model, we are able to halve the error and greatly reduce the variability in performance among predicted locations.

==> 6_etc/Acknowledgements_etc.tex <==
\paragraph{Acknowledgements}
We thank E. Kolibacz for his technical support. We are grateful to CityLab Berlin for providing their bike-sharing data. The European Union’s Horizon Europe research and innovation program funded this project under Grant Agreement No 101057131, Climate Action To Advance HeaLthY Societies in Europe (CATALYSE). Furthermore, the authors acknowledge support through the Emmy Noether grant KL 3037/1-1 of the German Research Foundation (DFG).

\paragraph{Author contributions}
S.K. designed the research, obtained the data, analyzed the data, and wrote the manuscript. L.K. conceived the research question, contributed materials, and co-wrote the paper. N.K. contributed materials and revised the paper.

\paragraph{Additional information}
Correspondence and requests for materials should be addressed to S.K. 

\paragraph{Competing interests}
The authors declare no competing interests.

\paragraph{Availability of code}
The code utilized for conducting the analysis and some exemplary data can be accessed through the following link: \href{https://drive.google.com/drive/folders/1cGa5di2SVGoKkmf8MdlGkpaPZG7TX43v?usp=sharing}{Link}. The code has been meticulously revised and tailored specifically for the submission of the paper, to be accessible to editors and reviewers during the review process. However, it is imperative to note that sharing this code with external entities is strictly prohibited until the paper undergoes publication. Furthermore, exemplar data has been made available, encompassing all pertinent features while presenting a limited set of observations. Notably, the Strava features within the dataset have been modified, due to the non-permissibility of public dissemination of this particular data.


==> Graphs/number_of_features.tex <==
231

==> packages.tex <==
% Language setting
\usepackage[english]{babel}

% Set page size and margins
\usepackage[a4paper,top=2cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

% For figures and graphics
\usepackage{graphicx}
\usepackage{svg} % for SVG images
\usepackage{subcaption}

% For tables
\usepackage{booktabs}
\usepackage{floatrow}
\usepackage{csvsimple}
%\usepackage{threeparttable}
\usepackage{tabularx}
\usepackage{longtable}
\usepackage{pdflscape}
\usepackage{colortbl}
\usepackage{booktabs}
\usepackage{threeparttable}

% For math and symbols
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}

% Threeparttable
%\usepackage{threeparttable}
% For hyperlinks
\usepackage[colorlinks=false, allcolors=black]{hyperref}

% For bibliographies
\usepackage[authoryear]{natbib}


% For footnotes under tables
\usepackage{caption}
\usepackage{makecell}
\renewcommand\theadfont{\bfseries}

% For line spacing
\usepackage[onehalfspacing]{setspace}

% For landscape pages
\usepackage{pdflscape}
\usepackage{lscape}

% For diagonal line in tables
\usepackage{slashbox}

% Control floats (graphs alone on page)
\renewcommand{\floatpagefraction}{.8}

% Line numbering
\usepackage{lineno}
%\linenumbers

% Indentation of first paragraph after section heading
\usepackage{indentfirst}

% Language setting
\usepackage[english]{babel}

%landscape 
\usepackage{pdflscape}

% fpr svg images
\usepackage{svg}

% Set page size and margins
\usepackage[a4paper,top=2cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

% for python tables
\usepackage{booktabs}
\usepackage{floatrow}

% to include csv files
\usepackage{csvsimple}

% Table float box with bottom caption, box width adjusted to content
\newfloatcommand{capbtabbox}{table}[][\FBwidth]
\usepackage{booktabs,caption}
\usepackage[flushleft]{threeparttable}

% Useful packages
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage[T1]{fontenc}
\usepackage{babel}

%subfigures
\usepackage{subcaption}

% for including to images 
\usepackage{graphicx}

% for mathsy signs
\usepackage{amssymb}
\usepackage{mathtools}
%\usepackage[colorlinks=true, allcolors=black]{hyperref}

% for stars * in tables
\usepackage{longtable}
\usepackage{threeparttablex} 
\usepackage{booktabs} 

% Useful packages
\usepackage{amsmath}
\usepackage{graphicx}

% line spacing
%\usepackage[singlespacing]{setspace}
 \usepackage[onehalfspacing]{setspace}
% \usepackage[doublespacing]{setspace}
 
% Bibliography
\usepackage[authoryear]{natbib}

% For flow charts
\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 

% For landscape pages
\usepackage{lscape}

% For footnote under tables
\usepackage{booktabs, caption, makecell}
\renewcommand\theadfont{\bfseries}
\usepackage{threeparttable}

% limit tables to textwidth
\usepackage{tabularx}
\usepackage{longtable}
\usepackage{pdflscape}
\usepackage{graphicx}

% control floats (graphs alone on page)
\renewcommand{\floatpagefraction}{.8}%

% Turn pages
\usepackage{rotating}

% to numerate lines
% \usepackage{lineno}
% \linenumbers

% ticks




%\usepackage[margin=1in,a4paper]{geometry} % page parameters
%\usepackage{longtable,booktabs,threeparttablex}
